SceneCrafter: Controllable Multi-View Driving Scene Editing

Simulation is crucial for developing and evaluating autonomous vehicle (AV) systems. Recent literature builds on a new generation of generative models to synthesize highly realistic images for full-stack simulation. However, purely synthetically generated scenes are not grounded in reality and have difficulty in inspiring confidence in the relevance of its outcomes. Editing models, on the other hand, leverage source scenes from real driving logs, and enable the simulation of different traffic layouts, behaviors, and operating conditions such as weather and time of day. While image editing is an established topic in computer vision, it presents fresh sets of challenges in driving simulation: (1) the need for cross-camera 3D consistency, (2) learning ``empty street" priors from driving data with foreground occlusions, and (3) obtaining paired image tuples of varied editing conditions while preserving consistent layout and geometry. To address these challenges, we propose SceneCrafter, a versatile editor for realistic 3D-consistent manipulation of driving scenes captured from multiple cameras. We build on recent advancements in multi-view diffusion models, using a fully controllable framework that scales seamlessly to multi-modality conditions like weather, time of day, agent boxes and high-definition maps. To generate paired data for supervising the editing model, we propose a novel framework on top of Prompt-to-Prompt to generate geometrically consistent synthetic paired data with global edits. We also introduce an alpha-blending framework to synthesize data with local edits, leveraging a model trained on empty street priors through novel masked training and multi-view repaint paradigm. SceneCrafter demonstrates powerful editing capabilities and achieves state-of-the-art realism, controllability, 3D consistency, and scene editing quality compared to existing baselines.

==> figures/fig_ablation.tex <==
\begin{figure}[t]
    \centering

\resizebox{\linewidth}{!}{
\begin{tikzpicture}

% Define image width, height, and vertical gap
\def\imagewidth{14.4cm}
\def\imageheight{1.8cm}
\def\verticalgap{-0.25cm} % Define the vertical gap as a variable

% First image
\node (image1) {\includegraphics[width=\imagewidth, height=\imageheight]{image_files/ablation_p2p/source.png}}; 
\node[anchor=east] at (image1.west) {Source}; 

% Second image
\node[below=\verticalgap of image1] (image2) {\includegraphics[width=\imagewidth, height=\imageheight]{image_files/ablation_p2p/nop2p.png}}; 
\node[anchor=east, align=right] at (image2.west) {Target}; 

% Third image
\node[below=\verticalgap of image2] (image3) {\includegraphics[width=\imagewidth, height=\imageheight]{image_files/ablation_p2p/cross_attn.png}}; 
\node[anchor=east, align=right] at (image3.west) {Target\\(w/ cross.)}; 

% Fourth image
\node[below=\verticalgap of image3] (image4) {\includegraphics[width=\imagewidth, height=\imageheight]{image_files/ablation_p2p/self_attn.png}}; 
\node[anchor=east, align=right] at (image4.west) {Target\\(w/ self.)};


\end{tikzpicture}
}

\caption{
\textbf{Ablation study on global edit paired data generation.}
Extending Prompt-to-Prompt~\cite{hertz2022prompt} to our setting with self-attention map manipulation allows us faithfully conduct the desired edit (to 7 PM) and still maintain the geometry structure to be consistent with the reference source images, while the other baselines failed.
}
\label{fig:ablation_p2p}
\end{figure}

==> figures/fig_compare.tex <==
\begin{figure}[t]
    \centering

\resizebox{\linewidth}{!}{
\begin{tikzpicture}

% Define image width, height, and vertical gap
\def\imagewidth{14.4cm}
\def\imageheight{1.8cm}
\def\verticalgap{-0.25cm} % Define the vertical gap as a variable

% First image
\node (image1) {\includegraphics[width=\imagewidth, height=\imageheight]{image_files/compare/gt_1.png}}; 
\node[anchor=east] at (image1.west) {Source}; 

% Second image
\node[below=\verticalgap of image1] (image2) {\includegraphics[width=\imagewidth, height=\imageheight]{image_files/compare/sdedit_1.png}}; 
\node[anchor=east, align=right] at (image2.west) {SDEdit~\cite{meng2021sdedit}}; 

% Third image
\node[below=\verticalgap of image2] (image3) {\includegraphics[width=\imagewidth, height=\imageheight]{image_files/compare/p2p_1.png}}; 
\node[anchor=east, align=right] at (image3.west) {P2P~\cite{hertz2022prompt}}; 

% Fourth image
\node[below=\verticalgap of image3] (image4) {\includegraphics[width=\imagewidth, height=\imageheight]{image_files/compare/ours_1.png}}; 
\node[anchor=east, align=right] at (image4.west) {SceneCrafter};


\end{tikzpicture}
}
\caption{
\textbf{Visual comparison on time of day editing.}
SceneCrafter is able to conduct realistic editing while still maintain the geometry structure of the input multi-view images.
\textit{Best viewed zoomed in.}
}
\label{fig:compare_time}
\end{figure}

==> figures/fig_gen.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.7\textwidth]{figures/gen.pdf}
    \caption{\textbf{Qualitative Results on Controllable Generation.} \zh{box, roadgraph, weather, time. each has two lines(Results and GT)}}
    \label{fig:gen}
\end{figure*}

==> figures/fig_teaser.tex <==

\begin{tikzpicture}

% Define image width, height, and vertical gap
\def\imagewidth{14.4cm}
\def\imageheight{1.8cm}
\def\verticalgap{-0.25cm} % Define the vertical gap as a variable

% First image
\node (image1) {\includegraphics[width=\imagewidth, height=\imageheight]{image_files/teaser/inpaint.png}}; 
\node[anchor=east] at (image1.west) {Original}; 

% Second image
\node[below=\verticalgap of image1] (image2) {\includegraphics[width=\imagewidth, height=\imageheight]{image_files/teaser/source.png}}; 
\node[anchor=east, align=right] at (image2.west) {Local Edit:\\Change Foreground}; 

% Third image
\node[below=\verticalgap of image2] (image3) {\includegraphics[width=\imagewidth, height=\imageheight]{image_files/teaser/weather.png}}; 
\node[anchor=east, align=right] at (image3.west) {Global Edit:\\Weather: Snowy}; 

% Fourth image
\node[below=\verticalgap of image3] (image4) {\includegraphics[width=\imagewidth, height=\imageheight]{image_files/teaser/time3.png}}; 
\node[anchor=east, align=right] at (image4.west) {Global Edit:\\Time: 7 PM};

% Draw arrows to connect one to another.
\draw[->, thick] (image1.east) to [out=-65,in=65] (image2.east); % Curved arrow
\draw[->, thick] (image2.east) to [out=-65,in=65] (image3.east); % Curved arrow
\draw[->, thick] (image3.east) to [out=-65,in=65] (image4.east); % Curved arrow

\end{tikzpicture}


